Software Resource Disaggregation for HPC with Serverless Computing

Aggregated HPC resources have rigid allocation systems and programming models which struggle to adapt to diverse and changing workloads. Consequently, HPC systems fail to efficiently use the large pools of unused memory and increase the utilization of idle computing resources. Prior work attempted to increase the throughput and efficiency of supercomputing systems through workload co-location and resource disaggregation. However, these methods fall short of providing a solution that can be applied to existing systems without major hardware modifications and performance losses. In this paper, we improve the utilization of supercomputers by employing the new cloud paradigm of serverless computing. We show how serverless functions provide fine-grained access to the resources of batch-managed cluster nodes. We present an HPC-oriented Function-as-a-Service (FaaS) that satisfies the requirements of high-performance applications. We demonstrate a software resource disaggregation approach where placing functions on unallocated and underutilized nodes allows idle cores and accelerators to be utilized while retaining near-native performance.

==> secs/background.bak.tex <==

Serverless provides an opportunity to bring elastic cloud programming models into high-performance
systems, as public clouds are not ready to accept HPC workloads.
%
FaaS provides a new resource allocation paradigm needed to resolve the issue of idle resources,
as a rigid system cannot handle large-scale and small-scale jobs without sacrificing memory
utilization (Sec.~\ref{sec:background_utilization_hpc}).
%
Functions can provide a software approach to fine-grained allocations of disaggregated
resources, overcoming the disadvantages and limitations of hardware solutions (Sec.~\ref{sec:background_resource_disaggregation}).
%
Simultaenously, functions can improve on the existing techniques and billing systems
for co-locating workloads (Sec.~\ref{sec:background_colocation}).
%
Finally, we discuss the characteristics of modern FaaS systems and limitations that prevent offloading
computations to idle and cheap resources (Sec.~\ref{sec:background_faas}).

%Our analysis is in line with past work. In four Lawrence Livermore National Laboratory (LANL) clusters,
%approximately 75% of the time, no more than 20% of memory is used [67]. Other work observed that many HPC
%applications use in the range of hundreds of MBs per computation core [85]. Interestingly, Alibaba’s published
%data [36] show that a similar observation is only true for machines that execute batch jobs, because batch jobs
%tend to be short and small. In contrast, for online jobs or co-located batch and online jobs, the minimum average
%machine memory utilization is 80%.
% 67 - On the Memory Underutilization: Exploring Disaggregated Memory on HPC Systems.
% 85 - Main Memory in HPC: Do We Need More or Could We Live with Less?
% 36 - Who Limits the Resource Eiciency of My Datacenter: An Analysis of Alibaba Datacenter Traces.
%
%In the MareNostrum supercomputer, the memory contributes 10\% of hardware cost
%and 10-15\% energy consumption~\cite{10.1145/3023362}.
%When scaling the application, the number of connections and messages increases,
%leading to increase in size of communication memory buffers~\cite{4215416} and network
%address mapping~\cite{7967191}.
\subsection{Utilization in HPC}
%
\label{sec:background_utilization_hpc}
%
Recent surveys indicate while a usage analysis of the Kraken
supercomputer capacity over a year indicates average utilization
as high as 94\%~\cite{10.1007/978-3-642-35867-8_14}, and a median utilization of around 90\%
on the Mira supercomputer~\cite{10.5555/3433701.3433812}, a four-year study of the Blue Waters system
capacity presents monthly utilization rates that rarely exceed 80\%~\cite{DBLP:journals/corr/JonesWIDSPGFSBK17}.
%
To assess the modern scale of the problem, we analyzed over a week the utilization of the Piz Daint
supercomputing system~\cite{pizDaint}, and present in Figures~\ref{fig:daint_cpu} and~\ref{fig:daint_memory}
the CPU and memory utilization data, respectively.
%
The rapid and frequent changes indicate that resources do not stay idle for an extended period of time,
and this gap cannot be addressed with persistent and long-running allocations.

HPC allocations tend to be compute-centric, and other resources such as memory and NIC are usually
assigned automatically and exclusively to allocated cores.
%
Multiple studies have examined memory and network utilization, indicating a vast resource
waste in the aggregated and statically allocated computing nodes.
%
At LLNL clusters, 90\% of jobs use less than 15\% of node memory, and 90\% of the time, node memory
utilization is less than 35\%~\cite{9235066}; high memory utilization occurs less than 2\% of the time~\cite{9235066}.
%
Four LANL clusters show average node memory usage of just 24\% and a huge discrepancy between
the 80th percentile and maximum memory use~\cite{10.1145/3352460.3358267}.
%
In the Cori supercomputer~\cite{10.1145/3514245}, node memory usage is not larger than 17.4\% of memory
for 75\% of the time, and 75\% of jobs never utilize more than 50\% of on-node memory.
%
% 0.46 GB/s, four DRAM modules per socket with 17 GB/s each - 0.67\%
Furthermore, the network and memory bandwidth utilization are bursty and very low most of the time -
75\% of the time, the memory and network bandwidth are no more than 0.67\% and 0.5\%, respectively.
%
NIC and memory bandwidth usage is bursty, and they can change significantly from near-idle value to almost a maximum.

Unfortunately, the problem of memory utilization is fundamentally not solvable with current static allocations
on homogenous resources because these do not represent the heterogeneity of HPC workloads.
%
When scaling, the memory per process usually decreases, and large-scale executions can need up
to 17x less memory per core~\cite{10.1145/3023362}.
%
While capacity computing applications with poor scaling require gigabytes of memory per process,
capability computing can use less than 10\% of available memory~\cite{10.1145/3023362}.
%
Furthermore, the discrepancy of memory footprint between master and worker processes
increases with scalability, up to 62.5x for some applications~\cite{10.1145/3023362}.
%
The memory on HPC nodes cannot be simply decreased because the High-Performance Linpack
needs at least 2 GB of memory per core to achieve maximum performance, and
this might rise to 16 GB on a system with million cores ~\cite{10.1145/3023362}.
%
With no remote memory available, nodes must be overprovisioned for the worst case, and
decreased memory would limit the maximal problem size that the system can handle.

Memory system contributes roughly 10 and 10-18\% of 
the capital and operational expenditures~\cite{10.1145/3023362,barroso2018datacenter}.
%
While turning off idle memory could decrease the static energy consumption~\cite{9235066},
it would also negatively affect memory parallelism~\cite{10.1145/3352460.3358267}.
%
Furthermore, it is not a long-term solution as the contribution of memory in energy usage of
a datacenter has been decreasing in the last years~\cite{barroso2018datacenter}.

\begin{bluebox}
HPC resources are heavily underutilized and overprovisioned.
%
Batch jobs cannot use the idle computing resources of their short availability,
and the diverse workloads force massive overprovisioning of memory. 
\end{bluebox}

\subsection{Resource Disaggregation}
\label{sec:background_resource_disaggregation}
%
Remote and disaggregated memory has been considered in data centers for
almost a decade now~\cite{10.1145/1555754.1555789,179767,201565,199305,10.1145/3127479.3131612}.
%
Disaggregation replaces overprovisioning for the worst case with allocating for the
average consumption but retaining the ability to expand memory dynamically.
%
Remote memory has been proposed for HPC systems~\cite{9235066},
but it comes with a bandwidth and latency penalty.
%
While modern high-speed networks allow retaining near-native performance in some applications~\cite{199305},
remote memory is considered challenging for fault tolerance, scalability, and performance reasons~\cite{10.1145/3127479.3131612}.
%Furthermore, remote memory problems increase keeping native application's performance requires high-speed interconnect
%with at most of 5 us of latency and up to 100 Gbps of bandwidth~\cite{199305},
%and memory bandwidth is the main reason for such requirements.

Furthermore, many disaggregation methods have not been adopted because of major investments needed~\cite{201565},
such as changes in the OS and hypervisor, explicit memory management, or hardware support
~\cite{4154093,10.1145/1555754.1555789,10.1145/1555754.1555789,9235066}.
%
Pricing models with dedicated memory billing are needed to avoid
throughput degradation in HPC systems with resource disaggregation~\cite{9652672}.
%
%  Existing applications and operating systems can directly benefit from
% our solution, without the need for modifications, custom
% middleware or intrusive OS extensions (e.g., swap and page
% fault -based data fetching). Furthermore, our approach uses
% a dedicated network to avoid impacting the main network
% latency with the traffic generated by memory disaggregation [29].
Hardware-level solutions can elevate performance issues, e.g., by providing
a dedicated high-speed network~\cite{10.1145/3127479.3131612}
and using dedicated memory blades~\cite{10.1145/1555754.1555789}.

\begin{bluebox}
Remote memory and resource disaggregation are not widely applied in HPC because of performance
overheads and increased complexity.
\end{bluebox}

%\subsection{Billing model}
%how does it impact HPC? describe batch systems
%disaggregation - describe disaggregation in cloud as a trend to treat CPU and memory differently
%say that clearly memory is underutilized - cite papers
%estimate the cost savings of having "regular" and "high-memory" nodes
%Very fine-grained multi-user access to the same resources
%what's the programming model? impact on BSP
%cite the Pueschel paper on variable thread level parallelism
%multi-tenancy - allocate high-memory, low-compute job with a reversed one
%measure memory, CPU and I/O utilization - try to find examples of application that show variation
%that we can use; memory not completely utilized, fill in something
%I don't want to scale my application because of CPU utilization, but I do this because of high
%memory footprint - I need to spread the ranks anyway. I'd like to allocate a lot of memory,
%run it on few cores and give more cores to someone else
%https://dl.acm.org/doi/10.1145/3023362

% The term symbiosis has been used to refer to the effectiveness with which multiple jobs achieve speedup when run on multithreaded machines [24] [25]. Symbiosis can be positive or negative. Jobs in an SMT processor can conflict with each other on various shared system resources. Throughput may go up or down depending on how well the jobs in the running set symbios or ‘get along’. It therefore makes a difference which jobs are coscheduled. A job scheduler which takes symbiosis into account can yield enhanced throughput and response time.
% Snavely, 2002
%
% Effects of contention and reduced memory bandwidth on performance can be estimated~\cite{10.1145/2155620.2155650,6494987}.
%
\subsection{HPC Co-location}
\label{sec:background_colocation}
%
Co-location helps to mitigate the underutilization problem by allowing more than one batch job
to run on the same node.
%
While some studies have not found a significant difference between node-sharing jobs
and exclusive jobs~\cite{10.1145/2616498.2616533,10.1145/2949550.2949553},
many applications experience significant performance degradation through contention in shared resources.
%
Prior work has attempted to improve scheduling on a node by detecting sharing and contention in memory bus,
bandwidth, and network interface~\cite{10.1145/511334.511343,10.1145/566726.566768,1655680,10.1145/1854273.1854306,1240622}.
%
When co-locating HPC workloads, it is essential to determine optimal \emph{node sharing} and \emph{partition} shared
resources.

in shared resources prefetchers, memory controllers, shared caches, network interface, memory bus, and even
the processor interconnect~\cite{10.5555/2388996.2389109,6468475}.

\textbf{Node sharing}
%
\emph{Symbiotic applications} can improve their performance when co-located
~\cite{10.1007/978-3-540-71035-6_10,10.1145/511334.511343,https://doi.org/10.1002/cpe.3187},
as long as they do not stress the same resources simultaneously.
%
In job stripping~\cite{https://doi.org/10.1002/cpe.3187}, combining processes
of different applications on shared resources helps reduce cache misses and network contention~\cite{5289162},
improving both node utilization and application's performance.
%
However, determining which workload pairs show positive symbiosis is not trivial.
%
Proposed methods include
characterization with the user hints and offline experiments~\cite{10.1007/978-3-540-71035-6_10,10.1145/1183401.1183450},
profiling and online monitoring~\cite{1655680,1240622,10.1145/2499368.2451126},
and machine learning~\cite{10.5555/2388996.2389109}.
%
For the co-location, systems can select applications with different characteristics~\cite{10.1007/978-3-540-71035-6_10,10.1145/1183401.1183450},
and use MPI communication patterns to avoid synchronized networking~\cite{5289162}.
%
Further benefits can be achieved with oversubscription
(node throughput up to 27\%~\cite{5470434}, system makespan up to 55\%~\cite{8547644}).

Another difficulty imposed by sharing is the unfairness of traditional billing models when applied
to jobs with performance impacted by the interference.
%
Alternative approaches include dedicated job queues with lower cost~\cite{https://doi.org/10.1002/cpe.3187}
and online detection of interference with price adjustment~\cite{6877470}.
%
Finally, default node sharing introduces security vulnerabilities unless tenants are isolated with
the help of containers and virtual machines.
%
When serverless functions are considered for co-location, the isolation is provided natively with the function sandbox,
while the fine-grained billing mechanism helps to charge users for resources used accurately.

\textbf{Partitioning}
%
Partitioning shared resources can reduce the effects of interference between co-located allocations.
%
Last-level cache (LLC) can be partitioned to co-locate latency-critical workloads while preserving
Quality of Service (QoS) guarantees~\cite{10.1145/2644865.2541944},
even at the cache line granularity~\cite{10.1145/2000064.2000073}.
%
The most efficient cache partitioning scheme can be found analytically for some applications~\cite{10.1145/2000064.2000073}.
%
Alternatively, partitioning can be made \emph{memory-aware} with the help of online monitoring and hardware solutions
by observing cache miss and hit rates~\cite{995703,4041865}, as not all applications use the cache
efficiently.
%
Memory bandwidth should be partitioned as well since cache contention is not the dominant factor
in performance degradation~\cite{10.1145/1736020.1736036}

Practical implementations of these techniques include Intel's Cache Allocation Technology (CAT)
and Memory Bandwidth Allocation (MBA)~\cite{intelCATMBA}.
%
Users can allocate cache size and memory bandwidth on a thread basis by using different
values of Class of Service (CLOS).
%
The bandwidth is controlled through the throttling of accesses that miss the L2 cache~\cite{10.1145/3337821.3337863}.
%
However, the throttling values expressed with CLOS are approximate.
%
Nevertheless, these technologies have already found applications in improving the efficiency and 
performance of co-scheduled applications~\cite{10.1145/3337821.3337863}.

\begin{bluebox}
  Node sharing is benefitial for performance and efficiency of HPC,
  as long as harmful interference is detected and mitigated.
  %
  Fine-grained and short functions can be good candidates for interference-aware co-location.
\end{bluebox}

\copik{citation for snapshotting}
\subsection{FaaS}
%
\label{sec:background_faas}
%
Serverless computing brings an abstract view of data center resources
allocated on the fly by the provider and hidden from the user.
%
The abstraction frees users from any responsibility for provisioning
and allows for elastic computing where users are billed only for resources used.
%
Function-as-a-Service is the dominating programming model for serverless where users program
and upload to the cloud stateless functions.
%
Here, we cover the most important limitations of serverless that are relevant for high-performance
computing.
%
For details on the implementation and particular challenges,
we refer to a discussion in the literature~\cite{DBLP:journals/corr/abs-1902-03383,copik2021sebs,10.5555/3277355.3277369}.

\textbf{Invocations}
%
Functions are invoked directly via an HTTP gateway, indirectly as a response to a cloud event,
and indirectly as a part of \emph{functions workflow}.
%
When an invocation is \emph{triggered}, the cloud system redirects
the request with a payload to a sandbox that can execute the function.
%
The rerouting is usually implemented with a centralized gateway~\cite{246288}, but decentralized
alternatives exist~\cite{copik2021rfaas}.
%
When no such sandbox is available, it is allocated and initialized executor process with the user's code.
%
This \emph{cold start} adds hundreds of milliseconds of overhead to the execution in the best
case~\cite{coldStart,10.1145/3423211.3425682}.
%
Providers attempt to minimize the frequency and severity of cold startups
by retaining containers during idle periods, prewarming containers, using lightweight virtual
machines, and snapshotting~\cite{216031,246288,10.1145/3373376.3378512}.
%
However, even a \emph{warm invocation} can introduce significant latencies when high-speed
network transport is not utilized~\cite{copik2021rfaas}.

% Parallelism of functions
%\textbf{Communication}
%%
%The communication between functions
%communication - P2P, Boxer, Roman's work. Others using collectives through storage - LambdaML, FK
%%

%
%New MPI standards and implementations have brought the benefits of emerging network protocols,
%above all with remote direct memory access (RDMA) networks such as InfiniBand~\cite{Liu2004}
%and the inclusion of RDMA programming through one-sided communication~\cite{fompi-mpi3-one-sided}.
%%
%%The RDMA systems offer a zero-copy and passive data transmission that entirely bypasses the operating system,
%%providing decreased CPU usage, lower latencies, and higher bandwidths.

%Related Work - some performance analysis has already been conducted:
%“Peeking Behind the Curtains of Serverless Platforms” @ ATC ‘18, they analyzed co-location, HW heterogeneity, performance isolation, I/O performance, and CPU utilization - but they measured this by checking how many CPU timeslots are assigned to a function? However, results are old (2017-2018) - we should reevaluate and compare.
%“Berkeley View of Serverless Computing” - analysis of compute-intensive workloads and their lack of performance and cost (high-level, few case studies).
%“Serverless Elastic Exploration of Unbalanced Algorithms”, CLOUD 2020 - Unbalanced Tree Search (UTS) and the Mandelbrot Set on Lambda vs Spark.
%“Towards Demystifying Serverless Machine Learning Training”, SIGMOD 2021 - analyze serverless from the ML perspective. Includes communication channels (Memcached, VM parameter servers, DynamoDB), performance \& cost evaluation + performance models (nice model FaaS vs IaaS in Sec 5.3).
%Our SeBS paper includes cost \& variability characterization.

\textbf{Serverless in HPC}
%
The elastic parallelism of FaaS has gained minor traction so far in the world of high-performance
and scientific computing~\cite{9284321}.
%
Still, serverless is used in compute-intensive workloads such as data analytics,
video encoding, linear algebra, and machine learning~\cite{227653,Mller2019LambadaID,
DBLP:journals/corr/abs-1907-11465,234886,DBLP:journals/corr/abs-1810-09679,10.1145/3357223.3362711,8360337,8457817,jiang2021towards}.
%
FaaS could implement the paradigm of \emph{evolving} jobs~\cite{10.1007/BFb0022284}
dispatching computations to newly allocated functions.
%
It could also implement \emph{malleable} jobs~\cite{10.1007/BFb0022284} by dynamically
changing the number of function executors when resource availability changes.
%
However, the applicability of serverless computing is limited by performance problems: high invocation
overheads, slow and expensive communication, lack of state and collective operations.
%
Invocations of fine-grained functions must come with a microsecond-scale latency.
%
Otherwise, the overhead of remote invocations can outweigh all benefits of computing with additional
resources (Sec.~\ref{sec:faas}).

Several systems have been proposed to address the limitations of serverless for high-performance
applications~\cite{funcx,nightcore,copik2021rfaas,10.5555/3277355.3277444,archipelago,wukong}.
%
However, they tend to focus on high-level optimizations of co-location, dynamic scheduling, and exploiting
intra-node communication.
%
Few systems support invocations with overhead lower than one millisecond~\cite{nightcore,copik2021rfaas}.
%
Furthermore, none of these systems comes with integration into batch systems and programming
paradigms common in HPC.

\begin{bluebox}
Serverless brings allocation and billing models needed in elastic and efficient computing.
%
Nevertheless, the adoption of serverless in HPC requires performance
improvements and a suitable programming model.
\end{bluebox}

% Notes

%Furthermore, on average three-quarters of node memory is not utilized~\cite{10.1145/3352460.3358267}.
%
%bandwidth and NIC bandwidth - bursts, but average is very underutilized
%
%18\% and 15\% of jobs request less than a full node on Stampede and Lonestar4, respectively~\cite{10.1145/2616498.2616533}.
%
%In the MareNostrum supercomputer, the memory contributes 10\% of hardware cost
%and 10-15\% energy consumption~\cite{10.1145/3023362}.
%
%Zivanovic et al.~\cite{10.1145/3023362} show that HPC nodes need at least 2 GB per core
%to allow applications such as the High-Performance Linpack to achieve high performance, which shows that memory
%cannot be simply decreased.
%%
%Furthermore, the required memory increases with the number of cores, predicting
%16 GB per core on a system with one million cores~\cite{10.1145/3023362}.
%%
%When scaling the application, the number of connections and messages increases,
%leading to increase in size of communication memory buffers~\cite{4215416} and network
%address mapping~\cite{7967191}.
%
%On the other hand, the memory per process often decreases when scaling applications,
%which means that large-scale and small-scale jobs might have widely different
%expectations on the available memory - up to 17x less memory needed~\cite{10.1145/3023362}.
%%
%Memory footprint depends on the HPC category of the application as well on its scalability~\cite{10.1145/3023362};
%capacity computing with limited scalability require gigabytes per process, whereas
%cabability computing application can use less than 10\% of memory when scaling.
%%
%FUrthermore, the discrepancy of memory footprint between master and worker processes
%increases with scalability, up to 62.5x for some applications~\cite{10.1145/3023362}.
%
%Analysis of four clusters in LANL~\cite{10.1145/3352460.3358267} show that average
%memory usage of a node is 24\%.
%%
%furthermore, there is a huge discrepancy -  the 80th percentile memory utilization 
%is around 20-30\%, but the max memory usage is above 70\%, with many nodes
%reaching 100\% utilization. Nodes must be overprovisioning for the worst case.
%%
%Otherwise we would decrease the maximal problem size that the system can handle,
%affecting significantly capacity computing.
%
%%Our analysis is in line with past work. In four Lawrence Livermore National Laboratory (LANL) clusters,
%%approximately 75% of the time, no more than 20% of memory is used [67]. Other work observed that many HPC
%%applications use in the range of hundreds of MBs per computation core [85]. Interestingly, Alibaba’s published
%%data [36] show that a similar observation is only true for machines that execute batch jobs, because batch jobs
%%tend to be short and small. In contrast, for online jobs or co-located batch and online jobs, the minimum average
%%machine memory utilization is 80%.
%% 67 - On the Memory Underutilization: Exploring Disaggregated Memory on HPC Systems.
%% 85 - Main Memory in HPC: Do We Need More or Could We Live with Less?
%% 36 - Who Limits the Resource Eiciency of My Datacenter: An Analysis of Alibaba Datacenter Traces.
%\todo{Cite datacenters}
%Michelogiannakis et al.~\cite{10.1145/3514245} conduct an analysis of the Cori supercomputer
%with 4GB of memory per core, four DRAM modules with a peak bandwidth of 17 GB/s per module.
%%
%An extensvie study of resurce utilization.
%%
%They show that that nodes use no more than 17.4\% of memory for three quarters of the time,
%and three quarters of jobs never utilize more than 50\% of on-node memory.
%%
%Three quarters of node use at most 0.46 GB/s of bandwidth.
%30.9\% of jobs never use more than 1GB/s of memory bandwidth per node, and the behavior can be bursty
%- high bandwidth uttilization for a short period of time.
%%
%Very low networ utilization - 75\% of time use no more than 0.5\% of NIC bandwidth.
%Also very bursty behavior.
%%
%NIC nad memory bandwidth can change significantly, from near-idle value to almost a maximum.
%
%ANalysis of production clusters and LLNL~\cite{9235066} shows that 90\% of jobs
%utilize less than 15\% of node memory, and 90\% of of the time, memory
%utilization is less than 35\%.
%%
%High utilization occurs rarely, less than 2\% of time.
%
%strong scaling - memory footprint changes significantly
%%
%Thus, large-scale and small-scale jobs cannot
%
%CPU - short time availability
%
%\subsection{Billing model}
%
%how does it impact HPC? describe batch systems
%
%disaggregation - describe disaggregation in cloud as a trend to treat CPU and memory differently
%
%say that clearly memory is underutilized - cite papers
%
%estimate the cost savings of having "regular" and "high-memory" nodes
%Very fine-grained multi-user access to the same resources
%
%what's the programming model? impact on BSP
%
%cite the Pueschel paper on variable thread level parallelism
%
%\copik{Does Daint allows to run two jobs on the same node?}
%multi-tenancy - allocate high-memory, low-compute job with a reversed one
%
%measure memory, CPU and I/O utilization - try to find examples of application that show variation
%that we can use; memory not completely utilized, fill in something
%
%I don't want to scale my application because of CPU utilization, but I do this because of high
%memory footprint - I need to spread the ranks anyway. I'd like to allocate a lot of memory,
%run it on few cores and give more cores to someone else
%https://dl.acm.org/doi/10.1145/3023362


% Notes resource disaggregation

%\textbf{Colocation}
%
%Co-located applications - memory contention between 10-60\% slowdown and
%"up to several orders of magnitude for I/O~\cite{10.1007/978-3-540-71035-6_10}
%
%Memory bus saturation causes up to 3-fold decrease in performance of bandwidth consuming applications~\cite{1240622}.
%
%Bandwidth is a precious resource in supercomputing systems - the bandwidth-per-flop ratio has been
%decreasing for the last decade~\cite{10.1145/3432261.3432263}.
%
%memory bandwidth requirements of applications are very different, a difference of a factor up to 4 times~\cite{1655680}.
%
%Priority scheduling for symbiotic multithreading computing, Snavely et al.~\cite{10.1145/511334.511343}.
%
%Profiling of MPI applications to detect applications which communication patterns are not
%synchronized to decrease network contention~\cite{5289162}.
%
%Liedtke et al.~\cite{10.1145/566726.566768} proposed memory bus scheduling to guarantee fairness
%for job mixes sharing the same memory bus across processors.
%
%Weinberg et al.~\cite{10.1007/978-3-540-71035-6_10,10.1145/1183401.1183450} propose a scheduler for space-sharing by using
%user input and experimentation to detect application characteristics and co-locate differnet classes of applications.
%
%Koukis et al.~\cite{1655680} propose an OS scheduler in SMP clusters to monitor NIC bandwidth between
%nodes and CPU memory bandwidth consumption within a node
%and use that to implement a memory bandwidth aware scheduler, decreasing contention on memory bus.
%
%bandwidth-aware job scheduling:  Xu et al.~\cite{10.1145/1854273.1854306} consider fine-granular fluctuations and show
%that even this changes have significant performance impact
%
%Antonopoulos et al.~\cite{1240622} propose to use performance monitoring counters to measure
%bandwidth consumption to co-locate processes that utilize fully bandwidth - but don't overutilize.
%
%Tang et al.~\cite{10.1145/2499368.2451126} uses PGO and dynamic monitoring to co-locate applications
%while preserving QoS guides.
%
%Machine learning method to predict contention effects when workloads are consolidated~\cite{10.5555/2388996.2389109}.
%
%
%\textbf{Paritioning}
%
%Kasture et al.~\cite{10.1145/2644865.2541944} propose a dynamic cache partitioning system for
%co-locating latency-critical workloads as the LLC is the resource that requires longest time to warm up
%and it degrades tail latency.
%Cache can be used to provide strict QoS guarantees on the tail latency.
%
%Cache partitioning can be applied at the cache line granularity~\cite{10.1145/2000064.2000073} with many partitions.
%
%Analytical model can be used to determine the mot efficient way of cache partitioning for concurrent tasks~\cite{10.1145/2000064.2000073}.
%
%Online monitoring and hardware solutions can be applied to determine if increasing cache partition size helps to increase
%cache hit rates~\cite{995703} - memory-aware partitioning.
%Also: give more cache parittion for an application that actually benefits from it instead of simply
%demanding it; a hardware circuit for monitoring and minimizing cache misses~\cite{4041865}.
%
%\textbf{Symbiosism}
%
%% The term symbiosis has been used to refer to the effectiveness with which multiple jobs achieve speedup when run on multithreaded machines [24] [25]. Symbiosis can be positive or negative. Jobs in an SMT processor can conflict with each other on various shared system resources. Throughput may go up or down depending on how well the jobs in the running set symbios or ‘get along’. It therefore makes a difference which jobs are coscheduled. A job scheduler which takes symbiosis into account can yield enhanced throughput and response time.
%% Snavely, 2002
%
%The idea of job stripping - spread two application processes across nodes 
%and combine them to benefit from different stressing of different reosurces - phases~\cite{https://doi.org/10.1002/cpe.3187}.
%
%Breslow et al.~\cite{https://doi.org/10.1002/cpe.3187} shows that combining processes
%of different applications on shared resources can help by reducing communication contention and
%reducing LLC misses.
%%
%Furthermore, the performacne can be predicted by examining application's when spreading.
%
%\textbf{Node sharing}
%%
%Iancu et al.~\cite{5470434} show that oversubscription on a shared multi-core server improves throughput
%by up to 27\% and can be an alternative to partitioning cores between applications.
%%
%Koop et al.~\cite{5289162} show that mixed workloads help to mitigate contention caused by synchronized
%networking and improve performance by up to 20\%.
%
%White et al.~\cite{10.1145/2616498.2616533} show that node sharing jobs do not show significant performance
%changes from interference when compared to node exclusive jobs on Stampede and Lonestar4 supercompusters
%- similar distributions of various HW metrics.
%%
%Further analysis with application kernels prove little interference, and reduced cache size
%has the highest effect on runtime of shared jobs~\cite{10.1145/2949550.2949553}.
%
%Xiong et al.~\cite{8547644} use oversubscription with node sharing to reduce makespan by up to 55\%.
%
%18\% and 15\% of jobs request less than a full node on Stampede and Lonestar4, respectively~\cite{10.1145/2616498.2616533}.
%
%\textbf{Fair Billing}
%%
%separated job queues for striped jobs with lower cost~\cite{https://doi.org/10.1002/cpe.3187}
%
%\textbf{Resource Disaggregation}
%%
%This doesn't work.
%%
%Disaggregation replaces overprovisioning for the worst case with provisioning for the
%average consumption, but retaining the ability to dynamically expand memory.
%%
%memory disaggregation for HPC~\cite{9235066} - bw and latency penalty.
%
%Remote and Disaggregated memory has been considered in datacenters for almost a decade now~\cite{10.1145/1555754.1555789,179767,201565,199305,10.1145/3127479.3131612}.
%%
%Many of these methods require new architectures, hardware support and dedicated
%programming models, inhibiting their adoption~\cite{201565}.
%%
%However, keeping native application's performance requires high-speed interconnect
%with at most of 5 us of latency and up to 100 Gbps of bandwidth~\cite{199305},
%and memory bandwidth is the main reason for such requirements.
%
%Methods - page swapping to remote memory~\cite{4154093,10.1145/1555754.1555789}, hardware-supported
%transparent and fine-grained access~\cite{10.1145/1555754.1555789}, and explicit
%user-space accessing of remote memory blocks~\cite{9235066}.
%%
%Infiniswap implements remote memory paging without modifications to the system~\cite{201565}.
%%
%Depending on the method, either OS and hypervisor modifications, explicit user management,
%or hardware support are needed.
%%
%They rely on the idea of oversubscribing memory resources and using methods
%such as page faults to redirect pages to remote memory.

